The Influence of Ridership Weighting on Targeting and Recovery Strategies for Urban Rail Rapid Transit Systems

The resilience of urban rapid transit systems (URTs) to a rapidly evolving threat space is of much concern. Extreme rainfall events are both intensifying and growing more frequent under continuing climate change, exposing transit systems to flooding, while cyber threats and emerging technologies such as unmanned aerial vehicles are exposing such systems to targeted disruptions. An imperative has emerged to model how networked infrastructure systems fail and devise strategies to efficiently recover from disruptions. Passenger flow approaches can quantify more dimensions of resilience than network science-based approaches, but the former typically requires granular data from automatic fare collection and suffers from large runtime complexities. Some attempts have been made to include accessible low-resolution ridership data in topological frameworks. However, there is yet to be a systematic investigation of the effects of incorporating low-dimensional, coarsely-averaged ridership volume into topological network science methodologies. We simulate targeted attack and recovery sequences using station-level ridership, four centrality measures, and weighted combinations thereof. Resilience is quantified using two topological measures of performance: the node count of a network's giant connected component (GCC), and a new measure termed the "highest ridership connected component" (HRCC). Three transit systems are used as case studies: the subways of Boston, New York, and Osaka. Results show that centrality-based strategies are most effective when measuring performance via GCC, while centrality-ridership hybrid strategies perform strongest by HRCC. We show that the most effective strategies vary by network characteristics and the mission goals of emergency managers, highlighting the need to plan for strategic adversaries and rapid recovery according to each city's unique needs.

==> supplementary_figures.tex <==

\begin{figure*}
  \includegraphics[width=\textwidth]{curves_attack_centrality_hrcc.png}
  \caption{Resilience curves  measured by HRCC (highest ridership in connected body) under attack by four centrality-based targeting strategies (Betweenness, Degree, Closeness, Eigenvector) and the mean of 500 random simulation curves with a 95\% confidence interval. From left to right: Boston T, Osaka Metro, New York City Subway.}
  \label{curvesattackcentralityhrcc}
\end{figure*}


\begin{figure*}
  \includegraphics[width=\textwidth]{curves_attack_hybrid_boston_4.1.png}
  \caption{Resilience curves for Boston MBTA network when under attack by ridership-based targeting, four hybrid strategies weighting ridership with each centrality (Betweenness-Hybrid, Degree-Hybrid, Closeness-Hybrid, Eigenvector-Hybrid), and the mean of 500 random simulation curves with a 95\% confidence interval. Left measures GCC (highest nodes in connected body), right measures HRCC (highest ridership in connected body).}
  \label{curvesattackhybridboston}
\end{figure*}


\begin{figure*}
  \includegraphics[width=\textwidth]{curves_attack_hybrid_newyork_4.3.png}
  \caption{Resilience curves for New York City Subway network when under attack by ridership-based targeting, four hybrid strategies weighting ridership with each centrality (Betweenness-Hybrid, Degree-Hybrid, Closeness-Hybrid, Eigenvector-Hybrid), and the mean of 500 random simulated curves with a 95\% confidence interval. Left measures GCC (highest nodes in connected body), right measures HRCC (highest ridership in connected body).}
  \label{curvesattackhybridnewyork}
\end{figure*}


\begin{figure*}
  \includegraphics[width=\textwidth]{curves_recovery_hrcc_boston_5.1.png}
  \caption{Resilience curves for Boston MBTA network by HRCC (highest ridership in connected body) during recovery phase. Left graph shows curves for four centrality-based attacking strategies (Betweenness, Degree, Closeness, Eigenvector), and right graph shows curves for ridership-based targeting, as well as four hybrid strategies weighting ridership with each centrality (Betweenness-Hybrid, Degree-Hybrid, Closeness-Hybrid, Eigenvector-Hybrid). Both graphs show the mean of 500 random simulated curves with a 95\% confidence interval.}
  \label{curvesrecoveryhrccboston}
\end{figure*}

\begin{figure*}
  \includegraphics[width=\textwidth]{curves_recovery_hrcc_osaka_5.2.png}
  \caption{Resilience curves for Osaka Metro network by HRCC (highest ridership in connected body) during recovery phase. Left graph shows curves for four centrality-based attacking strategies (Betweenness, Degree, Closeness, Eigenvector), and right graph shows curves for ridership-based targeting, as well as four hybrid strategies weighting ridership with each centrality (Betweenness-Hybrid, Degree-Hybrid, Closeness-Hybrid, Eigenvector-Hybrid). Both graphs show the mean of 500 random simulated curves with a 95\% confidence interval.}
  \label{curvesrecoveryhrccosaka}
\end{figure*}

